Fair Concurrent Training of Multiple Models in Federated Learning

Federated learning (FL) enables collaborative learning across multiple clients. In most FL work, all clients train a single learning task. However, the recent proliferation of FL applications may increasingly require multiple FL tasks to be trained simultaneously, sharing clients' computing and communication resources, which we call Multiple-Model Federated Learning (MMFL). Current MMFL algorithms use naive average-based client-task allocation schemes that can lead to unfair performance when FL tasks have heterogeneous difficulty levels, e.g., tasks with larger models may need more rounds and data to train. Just as naively allocating resources to generic computing jobs with heterogeneous resource needs can lead to unfair outcomes, naive allocation of clients to FL tasks can lead to unfairness, with some tasks having excessively long training times, or lower converged accuracies. Furthermore, in the FL setting, since clients are typically not paid for their training effort, we face a further challenge that some clients may not even be willing to train some tasks, e.g., due to high computational costs, which may exacerbate unfairness in training outcomes across tasks. We address both challenges by firstly designing FedFairMMFL, a difficulty-aware algorithm that dynamically allocates clients to tasks in each training round. We provide guarantees on airness and FedFairMMFL's convergence rate. We then propose a novel auction design that incentivizes clients to train multiple tasks, so as to fairly distribute clients' training efforts across the tasks. We show how our fairness-based learning and incentive mechanisms impact training convergence and finally evaluate our algorithm with multiple sets of learning tasks on real world datasets.

==> related.tex <==
\section{Background and Related Work}
Building on the literature on service and VM migration in follow-me-cloud \cite{TalebFollowMeCloud,SMfollowMeCloud}, 
\textbf{service or VM placement and migration} in light of user mobility in edge computing has been a widely studied problem \cite{wang2018survey,SWangSM_MDP, RLnetworkEdge, wang2019delay, OuyangFollowMe, networkAccessSP,ouyang2019adaptive, MSiew2021VM, kim2022modems}. 
These are often NP-hard knapsack-like problems.
In particular, \cite{SWangSM_MDP, wang2019delay} put forth an MDP formulation to make optimal migration decisions in light of unknown mobility information, with \cite{wang2019delay} using dynamic programming and reinforcement learning find the optimal solution.
\cite{OuyangFollowMe} optimized the performance-cost tradeoff in service migration in the long run via Lyapunov optimization.
\cite{networkAccessSP} formulated a joint network access and service placement problem.
\cite{ouyang2019adaptive} formulated a personalized performance service migration problem as a multi-armed bandit problem.
%These are often NP-hard knapsack-like problems, including cooperative edge caching~\cite{qiao2019deep}, demand aware VM migrations \cite{MSiew2021VM}, and mobility-aware VM migrations~\cite{kim2022modems}. 
%One of the challenges faced by such algorithms is ensuring they can adapt to new and unseen environments~\cite{wang2020fast} and that they can be trained rapidly~\cite{gerogiannis2022deep}. 
% \carlee{There are other papers here too (maybe cite a survey?) Talk about mobility as a challenge as it can create unpredictable dynamics (which leads into resilience).}
%\carlee{Find some papers on strict latency requirements for edge computing.}
Nevertheless, these service migration works have not approached the problem from the angle of resilience, preparing for and being adaptive to server failures.

At the same time, other works have realized that \textbf{cloud and edge computing presents resilience challenges}, particularly regarding resource allocation~\cite{shirazi2017extended}. Ultra-reliable offloading mechanisms have been proposed to address this challenge using two-tier optimization~\cite{liu2019dynamic}. %Migration itself can be a solution to edge server failures, if one can predict the failure in time to migrate or if the user does not store any state at the edge server~\cite{du2021optimal}. 
Proactive failure mitigation has also been proposed for edge-based NFV~\cite{huang2019proactive}. Failure aware workflow schedulling has been proposed for cloud computing \cite{cloudWorkflowSchedule}. Others have examined the use of reinforcement learning for replica placement in edge computing~\cite{liang2021two} and caching placement~\cite{zhang2020deep}. %\carlee{some of these works use multi-agent RL. It could be interesting to see how our resilience Q-learning interacts with that.}
The migration of users at overlapping coverage areas to other servers has been considered in \cite{du2021optimal}. Nevertheless, the users in the center of coverage areas still experience a higher latency, being connected the cloud under this scheme.
\cite{spatioTempFailTPDS} used graphical models to learn spatio-temporal dependencies between edge server and link failures. %, and hence service deployment combinations. 
Nevertheless, the above works did not consider resource allocation in light of unknown user mobility across different locations, or the cost of service migration.

\textbf{(Deep) reinforcement learning} has been used to optimize migration and offloading in edge computing, with the goal of minimizing migration costs and satisfying edge resource constraints while maximizing quality-of-computation~\cite{chen2018optimized,wang2019smart} or trading off the expended energy and latency~\cite{zhang2017energy}. %One of the challenges faced by such algorithms is ensuring they can adapt to new and unseen environments~\cite{wang2020fast}.
Importance sampling is widely used in reinforcement learning for policy evaluation (i.e., finding the expected future reward from following a given policy $\pi$) \cite{precup2000eligibility}, and prior work has proposed to utilize importance sampling to over-sample rare events for policy evaluation~\cite{frank2008reinforcement}. %\carlee{probably should talk about eligibility traces and the various RL papers we've been consulting here} 
However, these two works involve estimating the value function given a fixed policy, and does not consider learning the optimal policy $\pi^*$ which entails policy changes. Their proof techniques do not generalize to $Q$-learning; instead, our convergence proof is more similar to that of the convergence of $Q$-learning without importance sampling~\cite{sutton2018reinforcement}.
%While our proof is similar to that of tabular $Q$-learning without importance sampling~\cite{sutton2018reinforcement}, we must generalize it to incorporate the importance weights and show that the original bounds on various quantities used in the proof continue to hold.
Recent work has proposed using importance sampling to enhance RL's data efficiency~\cite{madhushani2020hamiltonian} in more general settings, but they do not consider rare events explicitly and use a more complex Hamiltonian Monte Carlo sampling technique that requires knowledge of the full system dynamics. %Thus, our convergence proof follows a simpler line of argument. 
%\carlee{Moreover, we further extend the traditional $Q$-learning convergence proofs to show that our convergence guarantees remain when using eligibility traces. I'm not sure if this is novel though?}

==> sections/algo_old_description.tex <==
\noindent\textbf{FedFairMMFL training (Algorithm~\ref{algo:FedFairMMFL}):} Our MMFL training proceeds in multiple rounds $t = 1,2,\ldots, T$. Let $\textbf{w}_s(t)$ denote the current global model of task $s$. In each round, the server first allocates clients to tasks (lines 4 to 6). %\carlee{
We let $Sel_s(t)$ denote the set of clients allocated to task $s$ in round $t$, dropping the subscript $s$ if it is clear from context. Following prior work on MMFL \cite{bhuyan2022multiProofs, bhuyan2022multi,liu2022multi}, we \textit{allocate each client to at most one task during each training round}, i.e., the $Sel_s(t)$ are disjoint across tasks $s$. For example, mobile clients \textcolor{violet}{or other resource constrained devices} may be performing other background tasks, e.g., running multiple applications, and thus may not have the computing power or battery to complete training rounds of multiple tasks. Allocating one task per client also reduces the communication overhead, as each client needs to receive only one updated global model in each global round. %We design a \textit{fair} task-client allocation method below. Some clients may not be allocated to any task; we call these \textit{inactive} clients.

Intuitively, uniform client-task allocation methods, like random or round robin allocation~\cite{bhuyan2022multi}, will train simpler tasks faster, since they allocate an equal number of clients to each task, in expectation.
%while more difficult models still remain at lower accuracies. 
%Therefore, in this work, we present an algorithm which \textbf{dynamically allocates tasks} to clients (during each local training iteration $t$), according to the real-time global accuracies (or losses) of the different models. 
We would instead like to ensure tasks are trained at more similar rates (i.e., achieve more fair performance) with a \textbf{difficulty-aware} client-task allocation algorithm, in which more users are allocated to tasks that currently have a higher loss compared to other tasks.
We can do so by inspecting the gradient of our MMFL objective in (\ref{eq:grad_g}). Since \textcolor{violet}{resource-constrained} clients can only compute gradients for one task per training round, we cannot exactly compute these gradients. Instead, we will assign each client to contribute to the gradient $\nabla F_{k,s}(\textbf{w}_s)$ for each task $s$ 
%in
\textcolor{red}{at a probability in proportion to its weight for that task}, i.e., proportional to $\alpha f_s(\textbf{w}_s)^{\alpha - 1} p_k$. We therefore allocate a task to each client according to the probability vector:
% \textcolor{blue}{As we are assigning one task per selected client each iteration, we make an approximation that instead of computing the full gradient (i.e., client $k$'s component of (\ref{eq:grad_g_full})), each client only works on the model which currently has the largest coefficient $q_tp_k f_{s}^{\alpha-1}$. When we set equal importance (same $q_t$) for all tasks, this is equivalent to each client being allocated to a task with the highest global loss}
%At each local training iteration, clients will be allocated tasks based on which task \textit{currently} has the highest global loss:
% \begin{equation}
%     \operatorname*{argmax}_{s \in \mathbb{S}} f^{\alpha-1}_s(w_s)
% \end{equation}
%\textcolor{blue}{ 
%To avoid being trapped in local minimum, e.g., in scenarios where the same clients constantly train the same model, we perform stochastic client-task allocation: Each client will be allocated a task based on this probability vector:}%To prevent the multiple model federated learning training process from being stuck at local minimum points, 
%we will add randomness in the client-task allocation process. At each local iteration, tasks will be selected for clients according to the following probabilities:
%\vspace{-1mm}
\begin{equation}
    %\textstyle
    \textbf{p}=\left[\frac{f^{\alpha-1}_1}{\sum_{s\in \mathbb{S}} f^{\alpha-1}_s}, \frac{f^{\alpha-1}_2}{\sum_{s\in \mathbb{S}} f^{\alpha-1}_s}, ..., \frac{f^{\alpha-1}_S}{\sum_{s\in \mathbb{S}} f^{\alpha-1}_s} \right],
    \label{eq:TaskAllocProbVec}
    %\vspace{-1mm}
\end{equation}
%The probability of being allocated to task $s$ is the ratio of the \textbf{current} $\alpha$-fair loss of task $s$, normalized.
Note that this allocation fulfills our intuition: \textbf{tasks with higher losses $f_s$ have a higher probability of being allocated clients.} 
\textcolor{blue}{For example, when $\alpha \rightarrow \infty$, \textit{all clients} will be allocated to the worst performing task, and when $\alpha=1$, allocation will be uniform.}
In Section~\ref{sec:fairConvgProofs}, we formalize this intuition by deriving a convergence bound for each task using FedFairMMFL. This selection scheme is \textit{unbiased} across clients: each client is equally likely to train a given task.

Given the clients allocated to each task $s$, the server then sends $\textbf{w}_s(t)$ to task $s$'s allocated clients (lines 5 to 8). Each active (i.e. available) client then trains its task on its corresponding local dataset by running $\tau$ SGD steps on the local loss $F_{k,s}$ of its assigned task $s$, as in traditional FL~\cite{mcmahan2017communication} (lines 10 to 15). Let $\textbf{w}_{k,s}(t)$ denote the updated local model for active client $k$ on its allocated task $s$.
%, and reduces the time spent waiting for stragglers.
Each active client then uploads $\textbf{w}_{k,s}(t)$ to the server, which aggregates the model parameters to synchronize the global model (lines 13 to 18). This aggregation uses weights $p_{k,Sel} = p_k/\sum_{k\in Sel} p_{k'}$ for each client $k$, where $Sel$ is the set of clients training task $s$ in this training round. The next training round then begins.

\begin{algorithm}[t]%[H]
	\caption{FedFairMMFL: Fair Training of Multiple Models in Federated Learning}
 \label{algo:FedFairMMFL}
 \small
	\begin{algorithmic}[1]
        \State \textbf{Initialization:} The global model weights $\textbf{w}_s$, for all tasks, \textcolor{violet}{initial random client-task allocation.}
		\For {$Global round =1,2,\ldots$}
            \For {all tasks $s$}
            \State \textcolor{brown}{Obtain global accuracy $f_s$ for all tasks $s \in \mathbb{S}$. }
                \State Server determines task allocation for clients, 
                \State based on $\mathbf{p}=\left[{f^{\alpha-1}_1}/{\sum_{s\in \mathbb{S}} f^{\alpha-1}_s}, ... \right]$ (Eq. \ref{eq:TaskAllocProbVec}).
                \State Server sends latest global model weights of task $s$, 
                \State $\textbf{w}_s$ to clients allocated.
            \EndFor
			\For {$clients=1,2,\ldots,K$}
                \If {Client $k$ is available for training this round}
    				%\State Client is allocated task $s$ based on $\mathbf{p}=\left[\frac{f^{\alpha-1}_1}{\sum_{s\in \mathbb{S}} f^{\alpha-1}_s}, ... \right]$ (Eq. \ref{eq:TaskAllocProbVec}).
                    %\State Server sends latest model weights of task $s$ to client.
                    \State Client performs local SGD (stochastic gradient descent) $\tau$ times for allocated 
                    task, optimizing $\textbf{w}_{k,s}$, and uploads $\textbf{w}_{k,s}$ to the server.
                \EndIf
			\EndFor
			\For{all tasks $s$} 
            \State Server aggregates 
           $\textbf{w}_s \gets \textbf{w}_s - \eta_t \sum_{k}  p_{k,Sel}  \nabla F_k(\textbf{w}_{s}) $. %q_s \alpha f^{\alpha-1}_s
            \EndFor
		\EndFor
	\end{algorithmic} 
\end{algorithm}
